Balanced spanning forests of graphs: Hardness and solving methods

The balanced connected $k$-partition problem (\textsc{bcp}) is a classic problem, which consists in partitioning the set of vertices of a vertex-weighted connected graph into a collection of~$k$ classes such that each class induces a connected subgraph of \emph{roughly} the same weight. In this study, we investigate edge-weighted variants of $\textsc{bcp}$, where, given a connected graph $G$, a positive integer $k$, and edge weights, the goal is to compute a spanning $k$-forest~$\mathcal{T}$ of $G$ (i.e., a forest with exactly $k$ trees) that minimizes the weight of the heaviest tree in~$\mathcal{T}$ in the min-max version, or maximizes the weight of the lightest tree in~$\mathcal{T}$ in the max-min version. We show that both versions of this problem are $\NP$-hard on complete graphs with $k=2$, unweighted split graphs, and unweighted bipartite graphs with $k\geq 2$ fixed. Moreover, we prove that these problems do not admit subexponential-time algorithms, unless the Exponential-Time Hypothesis fails. We focus on the min-max version and devise a tight $k$-approximation algorithm, compact and non-compact integer {linear programming} formulations, branch-and-cut, and branch-and-price algorithms. Finally, we present the outcomes of an experimental study on the performance of different solution methods. The source code of the complete implementation of the proposed algorithms is also available.

==> data-runtime-large-k.tex <==
% Columns: P total time, F total time, P solved, F solved.
% Solved flags for n>=30 come from recorded zero optimality gaps in Final-Results.xlsx.
% Existing n=20 times and classifications are retained.
7.04, 0.65, 1, 1
5.98, 0.73, 1, 1
6.13, 1.51, 1, 1
6.13, 0.66, 1, 1
6.21, 0.73, 1, 1
6.29, 1.48, 1, 1
6.32, 0.85, 1, 1
6.51, 1.04, 1, 1
5.94, 0.49, 1, 1
5.65, 0.54, 1, 1
6.22, 0.62, 1, 1
6.15, 0.51, 1, 1
6.27, 0.53, 1, 1
6.72, 0.41, 1, 1
6.19, 0.6, 1, 1
6.89, 0.86, 1, 1
7.21, 3.68, 1, 1
8.67, 1.68, 1, 1
8.1, 2.51, 1, 1
7.42, 3.29, 1, 1
7.55, 1.04, 1, 1
7.43, 0.8, 1, 1
7.82, 1.39, 1, 1
7.82, 0.83, 1, 1
7.92, 0.86, 1, 1
7.95, 0.94, 1, 1
7.76, 0.98, 1, 1
8.07, 1.11, 1, 1
8.53, 1.05, 1, 1
8.28, 0.79, 1, 1
8.04, 1.05, 1, 1
7.52, 0.71, 1, 1
9.97, 1.34, 1, 1
11.63, 1.99, 1, 1
9.63, 5.82, 1, 1
10.86, 3.75, 1, 1
10.72, 1.56, 1, 1
10.39, 1.34, 1, 1
10.14, 1.65, 1, 1
10.68, 1.2, 1, 1
9.5, 0.85, 1, 1
9.3, 1.06, 1, 1
9.62, 1.22, 1, 1
9.54, 1.09, 1, 1
10.57, 1.06, 1, 1
10, 0.84, 1, 1
10.66, 1.14, 1, 1
10.11, 1.06, 1, 1
12.3, 1.51, 1, 1
11.98, 1.39, 1, 1
11.38, 2.02, 1, 1
12.03, 2.39, 1, 1
11.66, 3.12, 1, 1
12.53, 1.12, 1, 1
11.54, 1.13, 1, 1
11.97, 0.96, 1, 1
10.86, 1.11, 1, 1
10.93, 1.13, 1, 1
11.26, 1.06, 1, 1
10.92, 0.97, 1, 1
11.53, 1.06, 1, 1
11.56, 1.1, 1, 1
12.04, 1.07, 1, 1
12.4, 1.06, 1, 1
8.24, 10.96, 1, 1
23.2, 4.24, 1, 1
6.83, 5.98, 1, 1
11.75, 6.78, 1, 1
45.98, 18, 1, 1
2.46, 2.68, 1, 1
4.83, 38.35, 1, 1
2.61, 5.39, 1, 1
2.12, 5.18, 1, 1
1.53, 1.79, 1, 1
5.42, 10.67, 1, 1
1.9, 3.03, 1, 1
1.24, 1.3, 1, 1
1.77, 1.86, 1, 1
2.26, 1.64, 1, 1
1.28, 1.31, 1, 1
9, 63.65, 1, 1
74.59, 24.44, 1, 1
24.27, 46.36, 1, 1
31.81, 37.39, 1, 1
18.67, 126.58, 1, 1
11.74, 50.52, 1, 1
4.36, 11.93, 1, 1
5.47, 20.17, 1, 1
1.32, 1.67, 1, 1
18.5, 239.76, 1, 1
13.82, 10.74, 1, 1
5.62, 36.42, 1, 1
2.06, 1.27, 1, 1
2.13, 1.28, 1, 1
9.96, 3.5, 1, 1
2.71, 1.63, 1, 1
875.67, 245.34, 1, 1
337.41, 966.38, 1, 1
78.71, 400.17, 1, 1
10.18, 2.42, 1, 1
113.54, 131.4, 1, 1
5.5, 22.74, 1, 1
24.77, 130.77, 1, 1
22.33, 237.32, 1, 1
18.18, 24.2, 1, 1
2.3, 2.19, 1, 1
19.74, 9.92, 1, 1
2.12, 4.71, 1, 1
2.7, 2.41, 1, 1
3.31, 1.38, 1, 1
13.82, 8.3, 1, 1
3.93, 1.84, 1, 1
690.88, 416.15, 1, 1
18.7, 18.16, 1, 1
190.76, 374.9, 1, 1
79.74, 37.74, 1, 1
4.08, 4.11, 1, 1
158.51, 38.97, 1, 1
7.61, 24.74, 1, 1
58.4, 183.07, 1, 1
49.32, 56.18, 1, 1
6.5, 240.53, 1, 1
2.45, 42.63, 1, 1
14.55, 32.39, 1, 1
10.47, 6.13, 1, 1
16.13, 15.45, 1, 1
8.35, 2.44, 1, 1
14.4, 1.56, 1, 1
47.09, 57.22, 1, 1
166.49, 459.03, 1, 1
150.49, 29.42, 1, 1
36.18, 471.95, 1, 1
66.31, 45.63, 1, 1
22.35, 202.21, 1, 1
18.14, 95.59, 1, 1
23.8, 72.9, 1, 1
23.13, 18.32, 1, 1
3.18, 6.61, 1, 1
2.96, 53.7, 1, 1
47.25, 109.71, 1, 1
1.79, 2.39, 1, 1
2.33, 8.82, 1, 1
1.27, 1.59, 1, 1
4.71, 2.9, 1, 1
384.56, 1014.7, 1, 1
7393.44, 107.84, 1, 1
435.51, 79.77, 1, 1
63.78, 592.83, 1, 1
114.36, 10801.58, 1, 0
494.45, 775.91, 1, 1
657.66, 4435.2, 1, 1
207.31, 3501.9, 1, 1
176.13, 10230.3, 1, 1
24.42, 137.25, 1, 1
39.02, 4754.59, 1, 1
23.14, 857.14, 1, 1
55.78, 431.22, 1, 1
165.84, 1223.8, 1, 1
28.98, 79.47, 1, 1
13.04, 4.21, 1, 1
1017.81, 7474.19, 1, 1
383.31, 1303.92, 1, 1
146.84, 129.9, 1, 1
80.36, 73.88, 1, 1
1678.47, 10811.56, 1, 0
1441.86, 10818.19, 1, 0
27.62, 2886.54, 1, 1
2374.83, 3461.96, 1, 1
181.94, 10805.82, 1, 0
191.02, 10810.64, 1, 0
116.74, 6030.09, 1, 1
133.66, 10822.29, 1, 0
3385.23, 1826.82, 1, 1
219.55, 8679.24, 1, 1
96.32, 7195.58, 1, 1
416.82, 6960.77, 1, 1
3623.22, 7991.05, 1, 1
432.89, 1827.37, 1, 1
273.55, 1033.43, 1, 1
10800, 9593.74, 0, 1
132.22, 2833.8, 1, 1
224.64, 10820.27, 1, 0
175.76, 10827.11, 1, 0
414.46, 10845.18, 1, 0
88.05, 10819.26, 1, 0
405.64, 10805.94, 1, 0
18.74, 1813.14, 1, 1
104.63, 10831.06, 1, 0
65.72, 1337.76, 1, 1
24.68, 10869.19, 1, 0
10800, 10816.51, 0, 0
981.27, 1680.38, 1, 1
131.55, 86, 1, 1
697.33, 1403.6, 1, 1
2064.55, 7777.91, 1, 1
379.87, 1573.67, 1, 1
1096.46, 1025.95, 1, 1
4250.43, 10821.42, 1, 0
230.8, 2380.2, 1, 1
35.26, 1471.37, 1, 1
232.43, 10869.55, 1, 0
1409.39, 10805.61, 1, 0
71.94, 1322.15, 1, 1
131.71, 10813.74, 1, 0
10800, 10816.5, 0, 0
67.45, 357.64, 1, 1
108.23, 10817.54, 1, 0
1944.05, 10815.42, 1, 0
2455.25, 1803.09, 1, 1
10800, 10488.46, 0, 1
10800, 2837.71, 0, 1
389.77, 2183.84, 1, 1
154.81, 1488.64, 1, 1
1387.65, 10803.43, 1, 0
10800, 10818.04, 0, 0
403, 10804.63, 1, 0
725.53, 10805.85, 1, 0
25.42, 10804.75, 1, 0
133.15, 10804.61, 1, 0
535.24, 10804.21, 1, 0
102.16, 10642.88, 1, 1
28.75, 402.31, 1, 1
159.63, 907.14, 1, 1
252.22, 10806.24, 1, 0
934.47, 6923.44, 1, 1
2365.74, 8978.32, 1, 1
487.93, 2109.44, 1, 1
835.13, 2173.84, 1, 1
7740.84, 10814.73, 1, 0
5788.35, 10823.86, 1, 0
4298.5, 10899.13, 1, 0
2008.74, 10829.24, 1, 0
708.61, 10814.96, 1, 0
205.97, 10827.73, 1, 0
10800, 10812.48, 0, 0
3823.57, 10904.5, 1, 0
1127.13, 10831.4, 1, 0
691.55, 10817.4, 1, 0
1422.58, 10833.68, 1, 0
948.69, 10831.07, 1, 0
1504.6, 7052.64, 1, 1
10800, 10894.7, 0, 0
882.48, 4933.73, 1, 1
10800, 10806.37, 0, 0
1187.6, 10910.41, 1, 0
10800, 10890.47, 0, 0
2237.81, 10819.12, 1, 0
10800, 10924.52, 0, 0
5355.89, 10893.27, 1, 0
10800, 10895.25, 0, 0
4519.41, 10827.34, 1, 0
1504.83, 10887.72, 1, 0
6205.9, 10828.13, 1, 0
480.61, 10827.04, 1, 0
3267.11, 10838.89, 1, 0
213.94, 10826.87, 1, 0
10800, 10817.36, 0, 0
10800, 10817.74, 0, 0
355.22, 6.74, 1, 1
5809.84, 1791.9, 1, 1
10800, 10815.98, 0, 0
951.59, 10900.2, 1, 0
8022.26, 10815.48, 1, 0
1081.05, 10817.27, 1, 0
10800, 10821.12, 0, 0
8443.68, 10820.34, 1, 0
441.3, 10818.03, 1, 0
915.96, 10809.89, 1, 0
1653.88, 10886.58, 1, 0
630.62, 10833.97, 1, 0
10596.27, 10829.33, 1, 0
2782.76, 10827.27, 1, 0
2399.05, 1458.59, 1, 1
2806.81, 7410.16, 1, 1
10800, 10809.25, 0, 0
10800, 10825.38, 0, 0
10800, 10813.21, 0, 0
10800, 10813.12, 0, 0
3295.5, 10817.14, 1, 0
546.47, 10814.81, 1, 0
710.3, 10828.7, 1, 0
1286.9, 10834.62, 1, 0
2539.11, 10833.07, 1, 0
927.52, 10819.81, 1, 0
293.3, 10843.03, 1, 0
10800, 10835.23, 0, 0
10800, 10902.55, 0, 0
865.17, 10843.33, 1, 0
1437.49, 1523.55, 1, 1
4423.32, 10804.71, 1, 0
9613.26, 10821.43, 1, 0
2478.78, 10855.69, 1, 0
8003.27, 10945.75, 1, 0
10800, 10817.95, 0, 0
10800, 8420.04, 0, 1
10800, 10821.87, 0, 0
10800, 10882.19, 0, 0
10800, 10821.15, 0, 0
1196.17, 10826.31, 1, 0
10800, 10828.04, 0, 0
10800, 10834.12, 0, 0
578.67, 10895.58, 1, 0
10800, 10823.35, 0, 0
1698.98, 10836.05, 0, 0


==> data-runtime-large-n.tex <==
% Columns: P total time, F total time, P solved, F solved.
% Solved flags for n>=30 come from recorded zero optimality gaps in Final-Results.xlsx.
% Existing n=20 times and classifications are retained.
21.73, 1.4, 1, 1
6.64, 1.96, 1, 1
10.29, 0.53, 1, 1
14.93, 0.68, 1, 1
8.24, 10.96, 1, 1
23.2, 4.24, 1, 1
6.83, 5.98, 1, 1
11.75, 6.78, 1, 1
45.98, 18, 1, 1
2.46, 2.68, 1, 1
4.83, 38.35, 1, 1
2.61, 5.39, 1, 1
2.12, 5.18, 1, 1
1.53, 1.79, 1, 1
5.42, 10.67, 1, 1
1.9, 3.03, 1, 1
1.24, 1.3, 1, 1
1.77, 1.86, 1, 1
2.26, 1.64, 1, 1
1.28, 1.31, 1, 1
7.62, 0.69, 1, 1
18.29, 0.98, 1, 1
161.08, 0.44, 1, 1
28.21, 0.43, 1, 1
9, 63.65, 1, 1
74.59, 24.44, 1, 1
24.27, 46.36, 1, 1
31.81, 37.39, 1, 1
18.67, 126.58, 1, 1
11.74, 50.52, 1, 1
4.36, 11.93, 1, 1
5.47, 20.17, 1, 1
1.32, 1.67, 1, 1
18.5, 239.76, 1, 1
13.82, 10.74, 1, 1
5.62, 36.42, 1, 1
2.06, 1.27, 1, 1
2.13, 1.28, 1, 1
9.96, 3.5, 1, 1
2.71, 1.63, 1, 1
61.91, 0.47, 1, 1
77.6, 5.13, 1, 1
35.48, 1.92, 1, 1
42.2, 0.89, 1, 1
875.67, 245.34, 1, 1
337.41, 966.38, 1, 1
78.71, 400.17, 1, 1
10.18, 2.42, 1, 1
113.54, 131.4, 1, 1
5.5, 22.74, 1, 1
24.77, 130.77, 1, 1
22.33, 237.32, 1, 1
18.18, 24.2, 1, 1
2.3, 2.19, 1, 1
19.74, 9.92, 1, 1
2.12, 4.71, 1, 1
2.7, 2.41, 1, 1
3.31, 1.38, 1, 1
13.82, 8.3, 1, 1
3.93, 1.84, 1, 1
42.24, 8.7, 1, 1
18.29, 1.42, 1, 1
48.97, 1.99, 1, 1
106.58, 5.17, 1, 1
690.88, 416.15, 1, 1
18.7, 18.16, 1, 1
190.76, 374.9, 1, 1
79.74, 37.74, 1, 1
4.08, 4.11, 1, 1
158.51, 38.97, 1, 1
7.61, 24.74, 1, 1
58.4, 183.07, 1, 1
49.32, 56.18, 1, 1
6.5, 240.53, 1, 1
2.45, 42.63, 1, 1
14.55, 32.39, 1, 1
10.47, 6.13, 1, 1
16.13, 15.45, 1, 1
8.35, 2.44, 1, 1
14.4, 1.56, 1, 1
84.42, 7.65, 1, 1
68.72, 1.89, 1, 1
223.57, 8.89, 1, 1
167.13, 2.61, 1, 1
47.09, 57.22, 1, 1
166.49, 459.03, 1, 1
150.49, 29.42, 1, 1
36.18, 471.95, 1, 1
66.31, 45.63, 1, 1
22.35, 202.21, 1, 1
18.14, 95.59, 1, 1
23.8, 72.9, 1, 1
23.13, 18.32, 1, 1
3.18, 6.61, 1, 1
2.96, 53.7, 1, 1
47.25, 109.71, 1, 1
1.79, 2.39, 1, 1
2.33, 8.82, 1, 1
1.27, 1.59, 1, 1
4.71, 2.9, 1, 1
161.21, 1.4, 1, 1
117.89, 2.22, 1, 1
153.59, 9.98, 1, 1
93.74, 6.51, 1, 1
384.56, 1014.7, 1, 1
7393.44, 107.84, 1, 1
435.51, 79.77, 1, 1
63.78, 592.83, 1, 1
114.36, 10801.58, 1, 0
494.45, 775.91, 1, 1
657.66, 4435.2, 1, 1
207.31, 3501.9, 1, 1
176.13, 10230.3, 1, 1
24.42, 137.25, 1, 1
39.02, 4754.59, 1, 1
23.14, 857.14, 1, 1
55.78, 431.22, 1, 1
165.84, 1223.8, 1, 1
28.98, 79.47, 1, 1
13.04, 4.21, 1, 1
1624.84, 4.7, 1, 1
10800, 11.19, 0, 1
222.77, 6.91, 1, 1
3443.35, 2.43, 1, 1
1017.81, 7474.19, 1, 1
383.31, 1303.92, 1, 1
146.84, 129.9, 1, 1
80.36, 73.88, 1, 1
1678.47, 10811.56, 1, 0
1441.86, 10818.19, 1, 0
27.62, 2886.54, 1, 1
2374.83, 3461.96, 1, 1
181.94, 10805.82, 1, 0
191.02, 10810.64, 1, 0
116.74, 6030.09, 1, 1
133.66, 10822.29, 1, 0
3385.23, 1826.82, 1, 1
219.55, 8679.24, 1, 1
96.32, 7195.58, 1, 1
416.82, 6960.77, 1, 1
898.82, 1.35, 1, 1
854.35, 4.48, 1, 1
10800, 9.87, 0, 1
1794.08, 10.57, 1, 1
3623.22, 7991.05, 1, 1
432.89, 1827.37, 1, 1
273.55, 1033.43, 1, 1
10800, 9593.74, 0, 1
132.22, 2833.8, 1, 1
224.64, 10820.27, 1, 0
175.76, 10827.11, 1, 0
414.46, 10845.18, 1, 0
88.05, 10819.26, 1, 0
405.64, 10805.94, 1, 0
18.74, 1813.14, 1, 1
104.63, 10831.06, 1, 0
65.72, 1337.76, 1, 1
24.68, 10869.19, 1, 0
10800, 10816.51, 0, 0
981.27, 1680.38, 1, 1
1691.84, 9.92, 1, 1
1115.39, 7.22, 1, 1
374.51, 3.46, 1, 1
242.5, 7.55, 1, 1
131.55, 86, 1, 1
697.33, 1403.6, 1, 1
2064.55, 7777.91, 1, 1
379.87, 1573.67, 1, 1
1096.46, 1025.95, 1, 1
4250.43, 10821.42, 1, 0
230.8, 2380.2, 1, 1
35.26, 1471.37, 1, 1
232.43, 10869.55, 1, 0
1409.39, 10805.61, 1, 0
71.94, 1322.15, 1, 1
131.71, 10813.74, 1, 0
10800, 10816.5, 0, 0
67.45, 357.64, 1, 1
108.23, 10817.54, 1, 0
1944.05, 10815.42, 1, 0
887, 11.99, 1, 1
128.66, 2.86, 1, 1
1347.72, 4.53, 1, 1
220.67, 20.66, 1, 1
2455.25, 1803.09, 1, 1
10800, 10488.46, 0, 1
10800, 2837.71, 0, 1
389.77, 2183.84, 1, 1
154.81, 1488.64, 1, 1
1387.65, 10803.43, 1, 0
10800, 10818.04, 0, 0
403, 10804.63, 1, 0
725.53, 10805.85, 1, 0
25.42, 10804.75, 1, 0
133.15, 10804.61, 1, 0
535.24, 10804.21, 1, 0
102.16, 10642.88, 1, 1
28.75, 402.31, 1, 1
159.63, 907.14, 1, 1
252.22, 10806.24, 1, 0
2721.75, 21.43, 1, 1
10800, 66.03, 0, 1
1697.59, 4.91, 1, 1
3579.4, 1.83, 1, 1
934.47, 6923.44, 1, 1
2365.74, 8978.32, 1, 1
487.93, 2109.44, 1, 1
835.13, 2173.84, 1, 1
7740.84, 10814.73, 1, 0
5788.35, 10823.86, 1, 0
4298.5, 10899.13, 1, 0
2008.74, 10829.24, 1, 0
708.61, 10814.96, 1, 0
205.97, 10827.73, 1, 0
10800, 10812.48, 0, 0
3823.57, 10904.5, 1, 0
1127.13, 10831.4, 1, 0
691.55, 10817.4, 1, 0
1422.58, 10833.68, 1, 0
948.69, 10831.07, 1, 0
1025.84, 3.85, 1, 1
5975.93, 17.84, 1, 1
559.16, 24.83, 1, 1
463.12, 2.86, 1, 1
1504.6, 7052.64, 1, 1
10800, 10894.7, 0, 0
882.48, 4933.73, 1, 1
10800, 10806.37, 0, 0
1187.6, 10910.41, 1, 0
10800, 10890.47, 0, 0
2237.81, 10819.12, 1, 0
10800, 10924.52, 0, 0
5355.89, 10893.27, 1, 0
10800, 10895.25, 0, 0
4519.41, 10827.34, 1, 0
1504.83, 10887.72, 1, 0
6205.9, 10828.13, 1, 0
480.61, 10827.04, 1, 0
3267.11, 10838.89, 1, 0
213.94, 10826.87, 1, 0
8126.71, 32.27, 1, 1
10624.59, 112.32, 1, 1
7141.8, 87.56, 1, 1
10800, 5.16, 0, 1
10800, 10817.36, 0, 0
10800, 10817.74, 0, 0
355.22, 6.74, 1, 1
5809.84, 1791.9, 1, 1
10800, 10815.98, 0, 0
951.59, 10900.2, 1, 0
8022.26, 10815.48, 1, 0
1081.05, 10817.27, 1, 0
10800, 10821.12, 0, 0
8443.68, 10820.34, 1, 0
441.3, 10818.03, 1, 0
915.96, 10809.89, 1, 0
1653.88, 10886.58, 1, 0
630.62, 10833.97, 1, 0
10596.27, 10829.33, 1, 0
2782.76, 10827.27, 1, 0
2428.29, 4.4, 1, 1
10800, 24.24, 0, 1
10800, 22.72, 1, 1
3002.49, 39.4, 1, 1
2399.05, 1458.59, 1, 1
2806.81, 7410.16, 1, 1
10800, 10809.25, 0, 0
10800, 10825.38, 0, 0
10800, 10813.21, 0, 0
10800, 10813.12, 0, 0
3295.5, 10817.14, 1, 0
546.47, 10814.81, 1, 0
710.3, 10828.7, 1, 0
1286.9, 10834.62, 1, 0
2539.11, 10833.07, 1, 0
927.52, 10819.81, 1, 0
293.3, 10843.03, 1, 0
10800, 10835.23, 0, 0
10800, 10902.55, 0, 0
865.17, 10843.33, 1, 0
3468.15, 8.78, 1, 1
1440.48, 78.18, 1, 1
4284.84, 5.55, 1, 1
10800, 1.83, 0, 1
1437.49, 1523.55, 1, 1
4423.32, 10804.71, 1, 0
9613.26, 10821.43, 1, 0
2478.78, 10855.69, 1, 0
8003.27, 10945.75, 1, 0
10800, 10817.95, 0, 0
10800, 8420.04, 0, 1
10800, 10821.87, 0, 0
10800, 10882.19, 0, 0
10800, 10821.15, 0, 0
1196.17, 10826.31, 1, 0
10800, 10828.04, 0, 0
10800, 10834.12, 0, 0
578.67, 10895.58, 1, 0
10800, 10823.35, 0, 0
1698.98, 10836.05, 0, 0


==> data-runtime.tex <==
% Columns: P total time, F total time, P solved, F solved.
% Solved flags for n>=30 come from recorded zero optimality gaps in Final-Results.xlsx.
% Existing n=20 times and classifications are retained.
12.54, 0.45, 1, 1
17.57, 0.43, 1, 1
14.67, 0.22, 1, 1
13.19, 0.19, 1, 1
7.04, 0.65, 1, 1
5.98, 0.73, 1, 1
6.13, 1.51, 1, 1
6.13, 0.66, 1, 1
6.21, 0.73, 1, 1
6.29, 1.48, 1, 1
6.32, 0.85, 1, 1
6.51, 1.04, 1, 1
5.94, 0.49, 1, 1
5.65, 0.54, 1, 1
6.22, 0.62, 1, 1
6.15, 0.51, 1, 1
6.27, 0.53, 1, 1
6.72, 0.41, 1, 1
6.19, 0.6, 1, 1
6.89, 0.86, 1, 1
32.95, 0.43, 1, 1
15.93, 0.21, 1, 1
19.23, 0.62, 1, 1
15.84, 0.16, 1, 1
7.21, 3.68, 1, 1
8.67, 1.68, 1, 1
8.1, 2.51, 1, 1
7.42, 3.29, 1, 1
7.55, 1.04, 1, 1
7.43, 0.8, 1, 1
7.82, 1.39, 1, 1
7.82, 0.83, 1, 1
7.92, 0.86, 1, 1
7.95, 0.94, 1, 1
7.76, 0.98, 1, 1
8.07, 1.11, 1, 1
8.53, 1.05, 1, 1
8.28, 0.79, 1, 1
8.04, 1.05, 1, 1
7.52, 0.71, 1, 1
13.77, 0.18, 1, 1
30.18, 0.3, 1, 1
24, 0.37, 1, 1
11.92, 0.21, 1, 1
9.97, 1.34, 1, 1
11.63, 1.99, 1, 1
9.63, 5.82, 1, 1
10.86, 3.75, 1, 1
10.72, 1.56, 1, 1
10.39, 1.34, 1, 1
10.14, 1.65, 1, 1
10.68, 1.2, 1, 1
9.5, 0.85, 1, 1
9.3, 1.06, 1, 1
9.62, 1.22, 1, 1
9.54, 1.09, 1, 1
10.57, 1.06, 1, 1
10, 0.84, 1, 1
10.66, 1.14, 1, 1
10.11, 1.06, 1, 1
26.02, 0.56, 1, 1
28.25, 0.59, 1, 1
17.55, 0.24, 1, 1
14.81, 0.18, 1, 1
12.3, 1.51, 1, 1
11.98, 1.39, 1, 1
11.38, 2.02, 1, 1
12.03, 2.39, 1, 1
11.66, 3.12, 1, 1
12.53, 1.12, 1, 1
11.54, 1.13, 1, 1
11.97, 0.96, 1, 1
10.86, 1.11, 1, 1
10.93, 1.13, 1, 1
11.26, 1.06, 1, 1
10.92, 0.97, 1, 1
11.53, 1.06, 1, 1
11.56, 1.1, 1, 1
12.04, 1.07, 1, 1
12.4, 1.06, 1, 1
21.73, 1.4, 1, 1
6.64, 1.96, 1, 1
10.29, 0.53, 1, 1
14.93, 0.68, 1, 1
8.24, 10.96, 1, 1
23.2, 4.24, 1, 1
6.83, 5.98, 1, 1
11.75, 6.78, 1, 1
45.98, 18, 1, 1
2.46, 2.68, 1, 1
4.83, 38.35, 1, 1
2.61, 5.39, 1, 1
2.12, 5.18, 1, 1
1.53, 1.79, 1, 1
5.42, 10.67, 1, 1
1.9, 3.03, 1, 1
1.24, 1.3, 1, 1
1.77, 1.86, 1, 1
2.26, 1.64, 1, 1
1.28, 1.31, 1, 1
7.62, 0.69, 1, 1
18.29, 0.98, 1, 1
161.08, 0.44, 1, 1
28.21, 0.43, 1, 1
9, 63.65, 1, 1
74.59, 24.44, 1, 1
24.27, 46.36, 1, 1
31.81, 37.39, 1, 1
18.67, 126.58, 1, 1
11.74, 50.52, 1, 1
4.36, 11.93, 1, 1
5.47, 20.17, 1, 1
1.32, 1.67, 1, 1
18.5, 239.76, 1, 1
13.82, 10.74, 1, 1
5.62, 36.42, 1, 1
2.06, 1.27, 1, 1
2.13, 1.28, 1, 1
9.96, 3.5, 1, 1
2.71, 1.63, 1, 1
61.91, 0.47, 1, 1
77.6, 5.13, 1, 1
35.48, 1.92, 1, 1
42.2, 0.89, 1, 1
875.67, 245.34, 1, 1
337.41, 966.38, 1, 1
78.71, 400.17, 1, 1
10.18, 2.42, 1, 1
113.54, 131.4, 1, 1
5.5, 22.74, 1, 1
24.77, 130.77, 1, 1
22.33, 237.32, 1, 1
18.18, 24.2, 1, 1
2.3, 2.19, 1, 1
19.74, 9.92, 1, 1
2.12, 4.71, 1, 1
2.7, 2.41, 1, 1
3.31, 1.38, 1, 1
13.82, 8.3, 1, 1
3.93, 1.84, 1, 1
42.24, 8.7, 1, 1
18.29, 1.42, 1, 1
48.97, 1.99, 1, 1
106.58, 5.17, 1, 1
690.88, 416.15, 1, 1
18.7, 18.16, 1, 1
190.76, 374.9, 1, 1
79.74, 37.74, 1, 1
4.08, 4.11, 1, 1
158.51, 38.97, 1, 1
7.61, 24.74, 1, 1
58.4, 183.07, 1, 1
49.32, 56.18, 1, 1
6.5, 240.53, 1, 1
2.45, 42.63, 1, 1
14.55, 32.39, 1, 1
10.47, 6.13, 1, 1
16.13, 15.45, 1, 1
8.35, 2.44, 1, 1
14.4, 1.56, 1, 1
84.42, 7.65, 1, 1
68.72, 1.89, 1, 1
223.57, 8.89, 1, 1
167.13, 2.61, 1, 1
47.09, 57.22, 1, 1
166.49, 459.03, 1, 1
150.49, 29.42, 1, 1
36.18, 471.95, 1, 1
66.31, 45.63, 1, 1
22.35, 202.21, 1, 1
18.14, 95.59, 1, 1
23.8, 72.9, 1, 1
23.13, 18.32, 1, 1
3.18, 6.61, 1, 1
2.96, 53.7, 1, 1
47.25, 109.71, 1, 1
1.79, 2.39, 1, 1
2.33, 8.82, 1, 1
1.27, 1.59, 1, 1
4.71, 2.9, 1, 1
161.21, 1.4, 1, 1
117.89, 2.22, 1, 1
153.59, 9.98, 1, 1
93.74, 6.51, 1, 1
384.56, 1014.7, 1, 1
7393.44, 107.84, 1, 1
435.51, 79.77, 1, 1
63.78, 592.83, 1, 1
114.36, 10801.58, 1, 0
494.45, 775.91, 1, 1
657.66, 4435.2, 1, 1
207.31, 3501.9, 1, 1
176.13, 10230.3, 1, 1
24.42, 137.25, 1, 1
39.02, 4754.59, 1, 1
23.14, 857.14, 1, 1
55.78, 431.22, 1, 1
165.84, 1223.8, 1, 1
28.98, 79.47, 1, 1
13.04, 4.21, 1, 1
1624.84, 4.7, 1, 1
10800, 11.19, 0, 1
222.77, 6.91, 1, 1
3443.35, 2.43, 1, 1
1017.81, 7474.19, 1, 1
383.31, 1303.92, 1, 1
146.84, 129.9, 1, 1
80.36, 73.88, 1, 1
1678.47, 10811.56, 1, 0
1441.86, 10818.19, 1, 0
27.62, 2886.54, 1, 1
2374.83, 3461.96, 1, 1
181.94, 10805.82, 1, 0
191.02, 10810.64, 1, 0
116.74, 6030.09, 1, 1
133.66, 10822.29, 1, 0
3385.23, 1826.82, 1, 1
219.55, 8679.24, 1, 1
96.32, 7195.58, 1, 1
416.82, 6960.77, 1, 1
898.82, 1.35, 1, 1
854.35, 4.48, 1, 1
10800, 9.87, 0, 1
1794.08, 10.57, 1, 1
3623.22, 7991.05, 1, 1
432.89, 1827.37, 1, 1
273.55, 1033.43, 1, 1
10800, 9593.74, 0, 1
132.22, 2833.8, 1, 1
224.64, 10820.27, 1, 0
175.76, 10827.11, 1, 0
414.46, 10845.18, 1, 0
88.05, 10819.26, 1, 0
405.64, 10805.94, 1, 0
18.74, 1813.14, 1, 1
104.63, 10831.06, 1, 0
65.72, 1337.76, 1, 1
24.68, 10869.19, 1, 0
10800, 10816.51, 0, 0
981.27, 1680.38, 1, 1
1691.84, 9.92, 1, 1
1115.39, 7.22, 1, 1
374.51, 3.46, 1, 1
242.5, 7.55, 1, 1
131.55, 86, 1, 1
697.33, 1403.6, 1, 1
2064.55, 7777.91, 1, 1
379.87, 1573.67, 1, 1
1096.46, 1025.95, 1, 1
4250.43, 10821.42, 1, 0
230.8, 2380.2, 1, 1
35.26, 1471.37, 1, 1
232.43, 10869.55, 1, 0
1409.39, 10805.61, 1, 0
71.94, 1322.15, 1, 1
131.71, 10813.74, 1, 0
10800, 10816.5, 0, 0
67.45, 357.64, 1, 1
108.23, 10817.54, 1, 0
1944.05, 10815.42, 1, 0
887, 11.99, 1, 1
128.66, 2.86, 1, 1
1347.72, 4.53, 1, 1
220.67, 20.66, 1, 1
2455.25, 1803.09, 1, 1
10800, 10488.46, 0, 1
10800, 2837.71, 0, 1
389.77, 2183.84, 1, 1
154.81, 1488.64, 1, 1
1387.65, 10803.43, 1, 0
10800, 10818.04, 0, 0
403, 10804.63, 1, 0
725.53, 10805.85, 1, 0
25.42, 10804.75, 1, 0
133.15, 10804.61, 1, 0
535.24, 10804.21, 1, 0
102.16, 10642.88, 1, 1
28.75, 402.31, 1, 1
159.63, 907.14, 1, 1
252.22, 10806.24, 1, 0
2721.75, 21.43, 1, 1
10800, 66.03, 0, 1
1697.59, 4.91, 1, 1
3579.4, 1.83, 1, 1
934.47, 6923.44, 1, 1
2365.74, 8978.32, 1, 1
487.93, 2109.44, 1, 1
835.13, 2173.84, 1, 1
7740.84, 10814.73, 1, 0
5788.35, 10823.86, 1, 0
4298.5, 10899.13, 1, 0
2008.74, 10829.24, 1, 0
708.61, 10814.96, 1, 0
205.97, 10827.73, 1, 0
10800, 10812.48, 0, 0
3823.57, 10904.5, 1, 0
1127.13, 10831.4, 1, 0
691.55, 10817.4, 1, 0
1422.58, 10833.68, 1, 0
948.69, 10831.07, 1, 0
1025.84, 3.85, 1, 1
5975.93, 17.84, 1, 1
559.16, 24.83, 1, 1
463.12, 2.86, 1, 1
1504.6, 7052.64, 1, 1
10800, 10894.7, 0, 0
882.48, 4933.73, 1, 1
10800, 10806.37, 0, 0
1187.6, 10910.41, 1, 0
10800, 10890.47, 0, 0
2237.81, 10819.12, 1, 0
10800, 10924.52, 0, 0
5355.89, 10893.27, 1, 0
10800, 10895.25, 0, 0
4519.41, 10827.34, 1, 0
1504.83, 10887.72, 1, 0
6205.9, 10828.13, 1, 0
480.61, 10827.04, 1, 0
3267.11, 10838.89, 1, 0
213.94, 10826.87, 1, 0
8126.71, 32.27, 1, 1
10624.59, 112.32, 1, 1
7141.8, 87.56, 1, 1
10800, 5.16, 0, 1
10800, 10817.36, 0, 0
10800, 10817.74, 0, 0
355.22, 6.74, 1, 1
5809.84, 1791.9, 1, 1
10800, 10815.98, 0, 0
951.59, 10900.2, 1, 0
8022.26, 10815.48, 1, 0
1081.05, 10817.27, 1, 0
10800, 10821.12, 0, 0
8443.68, 10820.34, 1, 0
441.3, 10818.03, 1, 0
915.96, 10809.89, 1, 0
1653.88, 10886.58, 1, 0
630.62, 10833.97, 1, 0
10596.27, 10829.33, 1, 0
2782.76, 10827.27, 1, 0
2428.29, 4.4, 1, 1
10800, 24.24, 0, 1
10800, 22.72, 1, 1
3002.49, 39.4, 1, 1
2399.05, 1458.59, 1, 1
2806.81, 7410.16, 1, 1
10800, 10809.25, 0, 0
10800, 10825.38, 0, 0
10800, 10813.21, 0, 0
10800, 10813.12, 0, 0
3295.5, 10817.14, 1, 0
546.47, 10814.81, 1, 0
710.3, 10828.7, 1, 0
1286.9, 10834.62, 1, 0
2539.11, 10833.07, 1, 0
927.52, 10819.81, 1, 0
293.3, 10843.03, 1, 0
10800, 10835.23, 0, 0
10800, 10902.55, 0, 0
865.17, 10843.33, 1, 0
3468.15, 8.78, 1, 1
1440.48, 78.18, 1, 1
4284.84, 5.55, 1, 1
10800, 1.83, 0, 1
1437.49, 1523.55, 1, 1
4423.32, 10804.71, 1, 0
9613.26, 10821.43, 1, 0
2478.78, 10855.69, 1, 0
8003.27, 10945.75, 1, 0
10800, 10817.95, 0, 0
10800, 8420.04, 0, 1
10800, 10821.87, 0, 0
10800, 10882.19, 0, 0
10800, 10821.15, 0, 0
1196.17, 10826.31, 1, 0
10800, 10828.04, 0, 0
10800, 10834.12, 0, 0
578.67, 10895.58, 1, 0
10800, 10823.35, 0, 0
1698.98, 10836.05, 0, 0

